Consensus-based Networked Tracking in Presence of Heterogeneous Time-Delays

We propose a distributed (single) target tracking scheme based on networked estimation and consensus algorithms over static sensor networks. The tracking part is based on linear time-difference-of-arrival (TDOA) measurement proposed in our previous works. This paper, in particular, develops delay-tolerant distributed filtering solutions over sparse data-transmission networks. We assume general arbitrary heterogeneous delays at different links. This may occur in many realistic large-scale applications where the data-sharing between different nodes is subject to latency due to communication-resource constraints or large spatially distributed sensor networks. The solution we propose in this work shows improved performance (verified by both theory and simulations) in such scenarios. Another privilege of such distributed schemes is the possibility to add localized fault-detection and isolation (FDI) strategies along with survivable graph-theoretic design, which opens many follow-up venues to this research. To our best knowledge no such delay-tolerant distributed linear algorithm is given in the existing distributed tracking literature.

==> 484.tex <==
%%% Note to Authors:
% Please read the following notices carefully before making any modification to the code. Thanks!
% 1) Do NOT change the sort of codes in anyway. For instance, dont move the ''\affiliation'' command above the ''\AddAuthor''.
% 2) There should be NO line breaks or blank lines between codes.
% 3) Do NOT delete the ''%'' sign at the end of lines.
% 4) If authors are all in a same institute, REMOVE the number next to the '\AddAuthor'' command (i.e., ''[1]'') and make sure there is only one ''\affiliation''.
% 5) Please write up to four clauses about your paper using ''\Item'' command. More items will be DELETED.
% 6) Make sure you will change the file name to your submission number. (for example ''315.tex'')
%
\Title{Consensus-based Networked Tracking in Presence of Heterogeneous Time-Delays}%
\AddAuthor[1]{Mohammadreza}{Doostmohammadian}%
\AddAuthor[2]{Mohammad}{Pirani}%
\AddAuthor[3]{Usman A.}{Khan}%
\affiliation[1]{School of Electrical Engineering, \\ \textit{Aalto University}, 
 Espoo, Finland, \\
\textit{Faculty of Mechanical Engineering}, \\
\textit{Semnan University}, Iran}%
\affiliation[2]{Mechanical and Mechatronics Engineering, \\
University of Waterloo, Canada}%
\affiliation[2]{Department of Electrical  Engineering, \\ 
Tufts University, Medford, MA, USA}%
\Targets{
\Item{This paper studies delay-tolerant distributed filtering strategies over a static sensor network subject to heterogeneous time-delays  and based on time-difference-of-arrival (TDOA) measurements. }%
\Item{The method is localized in the sense that a there is no single node of failure and the group of networked sensor networks locally (and collaboratively) detect the location of a mobile target with no need of a centralized coordinator.  }%
\Item{We proposed a linear TDOA measurement formulation that improves the existing nonlinear models in terms of accuracy and time-variance.   }%
\Item{This linear measurement model can be applied via other (both single and double time-scale) distributed estimation methods and can further be extended to consider localized FDI strategies and survivable network design.   }%
\figCaption{Delay-Tolerant Networked Estimation for Target Tracking }%
\endinput




